Polarization-Aware Ray-Tracing Enhanced Back-Projection Algorithm for Microwave Imaging in Complex Multipath Environments

A ray-tracing (RT) enhanced back-projection algorithm (RT-BPA) for microwave imaging in multipath environments is presented. By tightly incorporating the concept of ray-tracing into a generalized version of traditional BPA, this method ensures improved image quality by addressing two important issues. First, when the line-of-sight (LOS) path is obstructed, reflected paths, if available, enable imaging of hidden targets, which extends the applicability of the standard BPA beyond its normal use case. Second, the consideration of reflected ray-paths is equivalent to virtually increasing the aperture size, thus, improving image resolution without requiring new measurements. A key factor in achieving these advancements is the consideration of the vector nature of electromagnetic waves with polarization-dependent phase compensation, which is often ignored when employing a scalar-wave based formulation of the electromagnetic vector field. In addition, the presented method employs a shooting and bouncing rays (SBR) framework, offering better flexibility compared to manual path evaluation in existing RT-BPAs.

==> praemble/hft-macros-booktabs.tex <==
%% Booktabs

\newcolumntype {n}{c}
\newcolumntype {N}{>{\small}c}
\newcolumntype {L}{>{\small}l}
\newcolumntype {F}{>{\footnotesize}c}
\newcolumntype {v}[1]{>{\raggedright \hspace {0pt}} p {#1}}
\newcolumntype {V}[1]{>{\small \raggedright \hspace {0pt}} p {#1}}
\newcolumntype{d}[1]{>{\DC@{.}{.}{#1}}c<{\DC@end}}

\newcommand{\armultirow}[3]{%
    \multicolumn{#1}{#2}{%
        \begin{picture}(0,0)%
        \put(0,0){%
            \begin{tabular}[t]{@{}#2@{}}%
            #3%
            \end{tabular}%
        }%
        \end{picture}%
    }%
}%
% array.sty, rotating.sty
\newcolumntype{R}[1]{%
    >{\begin{turn}{90}\begin{minipage}{#1}\small\raggedright\hspace{0pt}}l%
            <{\end{minipage}\end{turn}}%
} 



==> praemble/hft-macros-environments.tex <==
\newcounter{subequation}
\newlength\mtabskip\mtabskip=-1.25cm
\renewcommand{\prec}{~\hat{<}~}
\newcommand\eqnCnt[1][]{ %
    \refstepcounter{subequation} %
    \begin{align}#1\end{align} %
    \addtocounter{equation}{-1}}
\def\mtabLong{long}
\makeatletter
\newenvironment{mtabular}[2][\empty]{ %
    \def\@xarraycr{ %
        \stepcounter{equation} %
        \setcounter{subequation}{0} %
        \@ifnextchar[\@argarraycr{\@argarraycr[\mtabskip]}}
    \let\theoldequation\theequation %
    \renewcommand\theequation{\theoldequation.\alph{subequation}}
    \edef\mtabOption{#1}
    \setcounter{subequation}{0} %
    \tabcolsep=0pt
    \ifx\mtabOption\mtabLong\longtable{#2}\else\tabular{#2}\fi %
}{ %
\ifx\mtabOption\mtabLong\endlongtable\else\endtabular\fi %
\let\theequation\theoldequation %
\stepcounter{equation}}
\makeatother

==> praemble/hft-macros-maths.tex <==
% Useful shortcuts
\newcommand{\mr}{\mathrm}
\newcommand{\ms}{\mathsf}
\newcommand{\mc}{\mathcal}
\newcommand{\wt}[1]{{\widetilde{#1}}}

\newcommand{\Or}[2]{\mc{O}{(#1)} + \mr{j} \mc{O}{(#2)}}

% Matrices, vectors, operators: shortcuts
\newcommand{\veg}[1]{\bm{#1}}     % geometrical / physical vectors
\newcommand{\vet}[1]{\bm{ \mathfrak{#1}}}    % I used it for physical vectors with time-dependency
\newcommand{\mat}[1]{\mathsfbfit{#1}} % n x n-dimensional matrix
\newcommand{\uv}[1]{\hat{\veg{#1}}} % unit vectors
\renewcommand{\vec}[1]{\mathsfbfit{#1}} %n-dimensional vector
\newcommand{\wvec}[1]{\widetilde{\mathsfbfit{#1}}} %widetilde n-dimensional vector
\newcommand{\wmat}[1]{\widetilde{\mathsfbfit{#1}}} %widetilde n-dimensional vector
\newcommand{\op}[1]{\mathcal{#1}} % operator that takes a scalar-valued function
\newcommand{\vecop}[1]{\bm{\mathcal{#1}}} % operator that takes a vector-valued function
\newcommand{\mel}[1]{\mathsfit{#1}} 
\newcommand{\vel}[1]{\mathsfit{#1}}
\newcommand{\matel}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\vecel}[1]{\begin{bmatrix} #1 \end{bmatrix}}

% Special matrices
\newcommand{\matI}{\mathbfsf{I}}
\newcommand{\matO}{\mathbfsf{0}}
\newcommand{\vecO}{\matO}
\newcommand{\vecI}{\mathbfsf{1}}


% Special geometrical vectors (mainly normals and unit vectors etc.)
\newcommand{\n}{\hat{\bm{n}}} 
\newcommand{\un}{\hat{\bm{u}}}
\newcommand{\np}{\hat{\bm{n}}^\prime}  
\newcommand{\pn}{\partial_{\hat{\bm{n}}}} 
\newcommand{\pnp}{\partial_{\hat{\bm{n}}^\prime}}  
\newcommand{\pnnp}{\partial_{\hat{\bm{n}},\hat{\bm{n}}^\prime}}    
\newcommand{\hek}{\hat{\bm{e}}_k}

% Real and imaginary part
\renewcommand{\Re}{\mathrm{Re}}
\renewcommand{\Im}{\mathrm{Im}}

% Differential symbol
\newcommand{\dd}{\mathrm{d}}  % The differential symbol is actually an operator

% Differential fractions
\newcommand{\ntfrac}[2]{\frac{\nt{#1}}{\nt{#2}}}  % partielles Differential
\newcommand{\pfrac}[2]{\frac{\uppartial #1}{\uppartial #2}}  % partielles Differential
\newcommand{\fracpd}[2]{\frac{\uppartial #1}{\uppartial #2}} % partielles Differential
\newcommand{\fracppd}[2]{\frac{\uppartial^2 #1}{\uppartial #2^2}}  % zweite partielle 
\newcommand{\fracd}[2]{\frac{\dd#1}{\dd #2}} % partielles Differential
\newcommand{\fracdd}[2]{\frac{\dd^2 #1}{\dd#2^2}}  % zweite partielle 

% Imaginary unit
\newcommand{\ii}{\mathrm{i}}   % For mathematicians and backwards compatibility
\newcommand{\im}{\mathrm{i}}  % For mathematician, Julia notation
\newcommand{\jm}{\mathrm{j}}  % For engineer stuff 

% Other math constants
\newcommand{\e}{\mathrm{e}}
\newcommand{\ep}{\varepsilon}
\newcommand{\sg}{\varsigma}

% Blackboard font: for special sets
\newcommand{\bbone}{\mathds{1}}  % mathds benötigt das Package "dsfont"
%\newcommand{\C}{\mathbb{C}}
\newcommand{\B}{B}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}

% Norms
%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}

% Math operators: analytic
\DeclareMathOperator{\hodge}{\mathbf{\upDelta}}
\DeclareMathOperator{\laplace}{\upDelta}
\DeclareMathOperator{\dirac}{\updelta}
\DeclareMathOperator{\dalembert}{\square}
\DeclareMathOperator{\ee}{e}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\tanc}{tanc}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\Rang}{Rang}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Null}{null}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\tr}{trace}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Eig}{Eig}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\vcurl}{\mathbf{curl}}
\DeclareMathOperator{\besselJ}{J}
\DeclareMathOperator{\besselN}{N}
\DeclareMathOperator{\hankel}{H}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
\DeclareMathOperator{\ricbessJ}{\mathbb{J}}
\DeclareMathOperator{\richankH}{\mathbb{H}}

% Math operators: linear algebra
\newcommand{\T}{\mr{T}}
\newcommand{\Ht}{\dagger}

% Math operators: special functions
\newcommand{\bJ}{\operatorname{J}}
\newcommand{\bH}{\operatorname{H}}
\newcommand{\bN}{\operatorname{N}}

% Math operation: restrain
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
        \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
        #1 % the function
        \vphantom{|} % pretend it's a little taller at normal size
        \right|_{#2} % this is the delimiter
}}


\newcommand\rst[3]{{% we make the whole thing an ordinary symbol
        \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
        #1 % the function
        \vphantom{|} % pretend it's a little taller at normal size
        \right|_{#2}^{#3} % this is the delimiter
}}

% Fourier transformations
\newcommand{\FT}{\cF}
\newcommand{\FTa}[1]{\cF\left[#1\right]}
\newcommand{\FTi}{\cF^{-1}}
\newcommand{\FTia}[1]{\cF^{-1}\left[#1\right]}

% Trace operators
\newcommand{\ttrace}{\upgamma_{\mathbf{t}}}
\newcommand{\Ntrace}{\upgamma_{\mathrm{N}}}

%
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

==> praemble/hft-macros.tex <==
\input{hft-macros-environments.tex} 
\input{hft-macros-maths.tex} 
\input{hft-packages-acro.tex} 
\input{hft-macros-booktabs.tex} 

% Other
\newcommand{\formatedtime}[3]{#1:#2:#3}
\newcommand{\formatedtimed}[4]{#1 days #2:#3:#4}

==> praemble/hft-packages-acro.tex <==
\usepackage{acro}

\DeclareAcronym{DG}
{
    short = DG ,
    long = discontinuous Galerkin
}


\DeclareAcronym{ACA}
{
    short = ACA ,
    long = adaptive cross approximation
}

\DeclareAcronym{EFIE}
{
    short =  EFIE ,
    long = electric field integral equation
}

\DeclareAcronym{MFIE}
{
    short =  MFIE ,
    long = magnetic field integral equation
}

\DeclareAcronym{CFIE}
{
    short =  CFIE ,
    long = combined field integral equation
}

\DeclareAcronym{MUIE}
{
    short =  MUIE ,
    long = Müller integral equation
}

\DeclareAcronym{PMCHWT}
{
    short =  PMCHWT ,
    long = Poggio-Miller-Chang-Harrington-Wu-Tsai integral equation
}

\DeclareAcronym{SPD}
{
    short =  SPD ,
    long = {symmetric, positive definite}
}

\DeclareAcronym{SPSD}
{
    short =  SPD ,
    long = {symmetric, positive semi-definite}
}

\DeclareAcronym{PEC}
{
    short =  PEC ,
    long = perfectly electrically conducting
}

\DeclareAcronym{RWG}
{
    short = RWG ,
    long = Rao-Wilton-Glisson
} 

\DeclareAcronym{BC}
{
    short = BC ,
    long = Buffa-Christiansen
} 


\DeclareAcronym{SVD}
{
    short = SVD ,
    long = singular value decomposition
} 


\DeclareAcronym{CG}
{
    short = CG ,
    long = conjugate gradient
} 

\DeclareAcronym{PCG}
{
    short = PCG ,
    long = preconditioned conjugate gradient
} 

\DeclareAcronym{CGS}
{
    short = CGS ,
    long = conjugate gradient squared
} 


\DeclareAcronym{CMP}
{
    short = CMP ,
    long = Calderón multiplicative preconditioner
} 

\DeclareAcronym{RFCMP}
{
    short = RF-CMP ,
    long = refinement-free Calderón multiplicative preconditioner
} 

\DeclareAcronym{HPD}
{
    short = HPD ,
    long = {Hermitian, positive definite}
} 

\DeclareAcronym{RHS}
{
    short = RHS ,
    long = right-hand side
}

\DeclareAcronym{LSE}
{
    short = LSE ,
    long = linear system of equations
}

==> praemble/hft-packages-cleveref.tex <==
\usepackage[english]{cleveref}

\Crefname{defn}{definition}{definitions}
\Crefname{defn}{Definition}{Definitions}

\Crefname{asm}{assumption}{assumptions}
\Crefname{asm}{Assumption}{Assumptions}

\crefname{lem}{lemma}{lemmas} 
\Crefname{lem}{Lemma}{Lemmas}

\crefname{prop}{proposition}{propositions} 
\Crefname{prop}{Proposition}{Propositions}

\crefname{thm}{theorem}{theorms} 
\Crefname{thm}{Theorem}{Theorms}

\crefname{cor}{corollary}{corollaries}
\Crefname{cor}{Corollary}{Corollaries}

==> praemble/hft-packages-review.tex <==
\usepackage{lineno}
\modulolinenumbers[5]
\usepackage{todonotes}
\usepackage{umoline}

\newcommand{\td}[1]{\todo[inline,size=\small]{#1}} % inline todo notes

==> praemble/hft-packages-theorem.tex <==
%%% Configure AMS MATH
\theoremstyle{definition}
\newtheorem{defn}{Definition}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}


==> praemble/hft-packages-tikz-pgfplots.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
% and optionally (as of Pgfplots 1.3):
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}
\newlength\figureheight
\newlength\figurewidth
\pgfplotsset{every axis plot/.append style={line width=1.5pt},
    legend style={font=\footnotesize, 
        text height=1.0ex,
        draw=black,
        fill=white,
        legend cell align=left}}


==> praemble/hft-paper-praemble-main.tex <==
\input{hft-paper-praemble-packages.tex}
\input{hft-macros.tex}
\input{sba-macros.tex}

==> praemble/hft-paper-praemble-packages.tex <==
% ill unnecessary alphabets
\newcommand{\hmmax}{0} 
\newcommand{\bmmax}{0} 

% Use UTF8
\usepackage[utf8]{luainputenc}

% Activate T1
\usepackage[T1]{fontenc}

\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}

% Ensure that we are language aware
\usepackage[english]{babel}
\addto\captionsenglish{\renewcommand{\figurename}{Fig.}}
\addto\captionsenglish{\renewcommand{\tablename}{Tab.}}
\usepackage{csquotes}

% Font stuff
\usepackage{newtxtext}
\usepackage{amsthm}
\usepackage[slantedGreek]{newtxmath}
%\usepackage{mathsfbf}
\usepackage[OMLmathsfit]{isomath}
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}
\usepackage{bm}
% Math packages
\usepackage{envmath}
\usepackage{mathtools}
\usepackage{commath}
%\usepackage{siunitx}
%\usepackage{amssymb} % SA: This package conflicts with the other font packages

% Figures
\usepackage[caption=false,font=footnotesize]{subfig}

% Tables
\usepackage{booktabs}
\usepackage{footmisc}  % Footnotes in floating environments

% Other
\usepackage{url}

\input{hft-packages-theorem.tex}
\input{hft-packages-review.tex}
\input{hft-packages-tikz-pgfplots.tex}
%\input{hft-packages-acro.tex}
%\usepackage{hyperref} % Load before cleveref
%\input{hft-packages-cleveref.tex}

==> praemble/sba-macros.tex <==
\NewDocumentCommand{\TA}{o}{
    \IfNoValueTF {#1} {%
        \vecop T_{\kern-2pt\mr{A}}
    }
    {
        \vecop T_{\kern-2pt\mr{A},#1}
    }
}

\NewDocumentCommand{\TPhi}{o}{
    \IfNoValueTF {#1} {%
        \vecop T_{\kern-2pt\Phiup}
    }
    {
        \vecop T_{\kern-2pt\Phiup,#1}
    }
}

\NewDocumentCommand{\matTA}{o}{
    \IfNoValueTF {#1} {%
        \mat T_\mr{A}   
        }
    {
        \mat T_{\mr{A},#1}
    }
}

\NewDocumentCommand{\matTPhi}{o}{
    \IfNoValueTF {#1} {%
        \mat T_\Phiup   
        }
    {
        \mat T_{\Phiup,#1}
    }
}

% Maxwell Single layer
\NewDocumentCommand{\MSL}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{SL}
        }
    {
        \veg \Psi_{\mr{SL},#1}
    }
}

% Maxwell Double layer
\NewDocumentCommand{\MDL}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{DL}
        }
    {
        \veg \Psi_{\mr{DL},#1}
    }
}

% vector Potential A
\NewDocumentCommand{\PA}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_\mr{A}
        }
    {
        \veg \Psi_{\mr{A},#1}
    }
}

% Maxwell Double layer
\NewDocumentCommand{\PPhi}{o}{
    \IfNoValueTF {#1} {%
        \veg \Psi_{\Phiup}
        }
    {
        \veg \Psi_{\Phiup,#1}
    }
}


%\newcommand{\TA}{\vecop T_{\kern-4pt\mr{A}}}
%\newcommand{\TPhi}{\vecop T_{\kern-4pt\Phiup}}

%\newcommand{\matTA}{\mat T_\mr{A}}
%\newcommand{\matTPhi}{\mat T_\Phiup}

\newcommand{\ZA}{\mat{Z}_\ms{A}}    
\newcommand{\ZPhi}{\mat{Z}_\ms{\Phi}}    

\newcommand{\matL}{\mat{\Lambda}}   
\newcommand{\matS}{\mat{\Sigma}}

\newcommand{\matLT}{\widetilde{\mat{\Lambda}}}   
\newcommand{\matST}{\widetilde{\mat{\Sigma}}}

\newcommand{\matLr}{\mat{\Lambda}_\ms{r}}
\newcommand{\matSr}{\mat{\Sigma}_\ms{r}}

\newcommand{\Pl}{\mat P_{\upLambda}}
\newcommand{\Ps}{\mat P_{\upSigma}}
\newcommand{\Pds}{\mat P_{\wt \upSigma}}
\newcommand{\Ph}{\mat P_{\mr H}}
\newcommand{\Plh}{\mat P_{\upLambda   \mr H}}
\newcommand{\Psh}{\mat P_{\upSigma   \mr H}}
\newcommand{\Pwl}{\wmat P_{\upLambda}}
\newcommand{\Pws}{\wmat P_{\upSigma}}
\newcommand{\Pwh}{\mat P_{\mr H}}
\newcommand{\Pwsh}{\wmat P_{\upSigma  \mr H}}

\newcommand{\hveg}[1]{\hat{\veg{#1}}}
\newcommand{\wveg}[1]{\widetilde{\veg{#1}}}

